TomasuLLM: Out-of-Order Speculative Execution for LLM Agents

Long-running tools can dominate coding-agent latency: compilers, test suites, and repository commands take seconds to minutes while the agent idles. This observation stall presents the same tension that drove out-of-order processors -- asequential interface hides work that can be predicted and started early, but a speculative result may become visible only after it and every earlier step have been validated. We present TomasuLLM, a runtime that executes agent tool calls out of trajectory order while preserving task-execution correctness. It drafts future actions, runs them in isolated copy-on-write sandboxes, traces their dependencies and effects, and commits results in trajectory order only after validation against committed state. Across three benchmarks spanning sub-second to minutes-long tool calls, TomasuLLM improves the reported benchmark means and scales with tool latency: 1.31x on 100 SWE-bench Verified tasks, 1.35x on 28 Terminal-Bench 2.0 tasks, and 1.27x matched progress on 18 SWE-Marathon sessions. Across 4,010 audited commit-validation records, it produces zero false accepts.

==> tables/eval_correctness_generated.tex <==
\begin{tabularx}{\columnwidth}{@{}l c c c c@{}}
\toprule
Validation rule & Records & Trace check & State/effect eq. & False accepts \\
\midrule
\texttt{read} & 1600 & 100\% & 100\% & 0\\
\texttt{write}/\texttt{edit} & 800 & 100\% & 100\% & 0\\
\texttt{bash} read-only & 640 & 99\% & 100\% & 0\\
test/compile & 580 & 98\% & 100\% & 0\\
speculation barrier & 390 & 100\% & 100\% & 0\\
\bottomrule
\end{tabularx}


==> tables/eval_cost_generated.tex <==
% Auto-generated by figures/plot_eval_audit_tables.py -- do not edit by hand.
\begin{tabularx}{\columnwidth}{@{}X r r@{}}
\toprule
Per-task average & Serial Pi & \system{} \\
\midrule
Main-agent tokens (M) & 8.2 & 8.3 \\
Drafter tokens (M) & 0 & 1.6 \\
Drafter GPU-seconds & 0 & 1{,}480 \\
Sandbox CPU-seconds & 2{,}760 & 4{,}310 \\
Wasted speculative tool-seconds & 0 & 128 \\
Speculative compute per second saved (s) & -- & 2.1 \\
\bottomrule
\end{tabularx}


==> tables/eval_outcome_generated.tex <==
% Auto-generated by figures/plot_eval_audit_tables.py -- do not edit by hand.
\begin{tabularx}{\columnwidth}{@{}X c c c@{}}
\toprule
Outcome (of 18 tasks) & Serial Pi & \system{} & $\Delta$ \\
\midrule
Pass & 1 & 1 & 0 \\
Fail & 11 & 11 & 0 \\
Timeout & 6 & 6 & 0 \\
\midrule
Completed within budget & 12 & 12 & 0 \\
\bottomrule
\end{tabularx}

